Short distance behaviour of the effective string

We study the Polyakov loop correlator in the (2+1) dimensional Z_2 gauge model. An algorithm that we have presented recently, allows us to reach high precision results for a large range of distances and temperatures, giving us the opportunity to test predictions of the effective Nambu-Goto string model. Here we focus on the regime of low temperatures and small distances. In contrast to the high temperature, large distance regime, we find that our numerical results are not well described by the two loop-prediction of the Nambu-Goto model. In addition we compare our data with those for the SU(2) and SU(3) gauge models in (2+1) dimensions obtained by other authors. We generalize the result of L\"uscher and Weisz for a boundary term in the interquark potential to the finite temperature case.

==> bound_app.tex <==
%%%%%%%%   FIRST REVISED VERSION
%%%%%%%%   MARCO, MAY 12TH
%%%%%%%%
%%%%%%%%
\newpage
\appendix{}
\label{app}
\vskip 0.5cm
\section{{{Evaluation of the functional form of the boundary correction.}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\theequation}{A.\arabic{equation}}
\setcounter{equation}{0}


Let us begin by considering the case when we assume
that the dynamics of the effective
string world sheet is described by a pure Nambu--Goto
action, neglecting a possible boundary term: under this
hypothesis, the action is given by the string world
sheet surface area (measured in units of the inverse
string tension), and the expectation value for the Polyakov
loop correlator can be expressed as
the partition function:
\eq
\label{partitionfunction}
Z= \int \left[ \mathcal{D} h \right] e^{-\sigma \mathcal{A}_0}
\qe
The Nambu--Goto action
$\mathcal{A}_0$ can be written in the following form:
\eq
\label{nambugoto}
\mathcal{A}_0 = \int_0^R \!\!\! dz \int_0^L \!\!\! dt
\sqrt{\det g_{\alpha \beta}}
\qe
where $g_{\alpha \beta}$ is defined as:
\eq
\label{g}
g_{\alpha \beta} = \partial_\alpha X^\mu\partial_\beta X_\mu
\en
Let us focus on the case of three dimensions:
we can parametrize the $X$ field in the
following way:
\eqa
\label{parametrizzazione}
X_1&=&z; \\ \nonumber
X_2&=&t; \\ \nonumber
X_3&=&h \;\;=\;\; h\left(z,t\right); \\
\ena
and the $h$ field is associated to the string world sheet
surface transverse displacement with respect to a minimal area
plane. Thus we have:
\eq
\label{nambugoto3d}
\mathcal{A}_0 = \int_0^R \!\!\! dz \int_0^L \!\!\! dt
\sqrt{1 + \left( \frac{\partial h}{\partial z} \right)^2
+\left( \frac{\partial h}{\partial t} \right)^2}
\en
A Taylor expansion of the square root
appearing in Eq. (\ref{nambugoto3d})
gives --- to first non-trivial order:
\eq
\label{aquadratica}
\mathcal{A}_0 \simeq \int_0^R \!\!\! dz \int_0^L \!\!\! dt
\left\{
1+\frac{1}{2} \left[ \left( \frac{\partial h}{\partial z} \right)^2
+\left( \frac{\partial h}{\partial t} \right)^2 \right]
\right\}
\en
and the partition function can be approximated as:
\eq
\label{z0+1}
Z_{0+1}= e^{-\sigma RL} \int \left[ \mathcal{D} h \right]
e^{-\frac{\sigma}{2} \int_0^R \!\!\! dz \int_0^L \!\!\! dt
\left[ \left( \frac{\partial h}{\partial z} \right)^2
+\left( \frac{\partial h}{\partial t} \right)^2 \right]}
\en
On the other hand, if we allow for the existence of a possible ``boundary
term'', the effective action will take the form:
\eq
\label{zstar}
Z^\star = \int \left[ \mathcal{D} h \right] e^{-\sigma \mathcal{A}}
\en
with:
\eq
\label{a}
\mathcal{A}=\mathcal{A}_0 +\frac{b}{4} \int_0^L \!\!\! dt
\left[  \left( \frac{\partial h}{\partial z} \right)_{z=0}^2
+  \left( \frac{\partial h}{\partial z} \right)_{z=R}^2
\right]
\en
where $b$ is a parameter with dimensions $[\mbox{length}]$,
while 
the $\frac{1}{4}$ factor is just a conventional 
choice (see also \cite{lw02}).\\
Let us notice that, in the case of the system we are
presently interested in, namely: a finite
temperature confining gauge theory\footnote{The string world sheet
associated to the expectation value of the Polyakov
loop correlator in a finite temperature gauge theory
is characterized by fixed boundary conditions in the
$z$ direction, and periodic boundary conditions
in the compactified, $t$ direction.}, the $z$-dependence of 
the eigenfunctions appropriate to the case of the pure
Nambu--Goto action can be factored out as:
\eq
\label{zdependence}
\sin \left( \frac{n\pi z}{R} \right)  \;\;\; , \;\;\;n \in \mathbf{N}_0
\en
thus:
\eq
\label{autovalori}
\frac{\partial h}{\partial z}= \frac{n\pi}{R} \cos \left(
\frac{n\pi z}{R} \right) \dots
\en
where we omitted the eigenfunction term
expressing the $t$-dependence; thus we have:
\eqa
\label{autovaloriin0er}
\left( \frac{\partial h}{\partial z} \right)_{z=0}^2 \!\!\!\!\!\!&=&\!\!
\left( \frac{\partial h}{\partial z} \right)_{z=R}^2 =
\frac{n^2 \pi^2}{R^2} \left. \cos^2 \left( \frac{n\pi z}{R}
\right) \right|_{z=0} \dots =
\frac{n^2 \pi^2}{R^2} \left. \cos^2 \left( \frac{n\pi z}{R}
\right) \right|_{z=R} \dots \nonumber \\
\!\!\!&=&\!\! \frac{n^2 \pi^2}{R^2} \dots
\ena
As it is concerned with the momentum in the compactified
direction, the eigenvalues are:
\eq
\label{autovalorit}
\frac{4\pi^2 m^2}{L^2} \;\;\; , \;\;\;m \in \mathbf{Z}
\en
If we define:
\eq
\label{rhotau}
\left\{
\begin{array}{c}
\rho = R \\
\tau = \frac{L}{2}
\end{array}
\right.
\en
the eigenvalues of the $(-\Delta)$ operator can be written as:
\eq
\label{autovalori-lapl}
\pi^2 \left( \frac{n^2}{\rho^2} + \frac{m^2}{\tau^2} \right)
\qe
Taking into account the boundary term too, the
complete action $\mathcal{A}$ reads, to first non-trivial order:
\eqa
\label{acompletaquadratica}
\mathcal{A} \simeq & & \!\!\!\!\!\!\!\! \int_0^R \!\!\! dz \int_0^L \!\!\! dt
\left\{
1+\frac{1}{2} \left[ \left( \frac{\partial h}{\partial z} \right)^2
+\left( \frac{\partial h}{\partial t} \right)^2 \right]
\right\} \nonumber \\ 
& &+ \frac{b}{4} \int_0^L \!\!\! dt
\left[  \left( \frac{\partial h}{\partial z} \right)_{z=0}^2 \!\!\!\!
+  \left( \frac{\partial h}{\partial z} \right)_{z=R}^2
\right]
\ena
Now, we propose to work out the correction to the 
$V(R)$ interquark potential to first order in $b$ 
in a perturbative expansion; to do this, we have to 
evaluate:
\eq
\label{z01}
Z_{0+1}^\star = \left[  \int \left[ \mathcal{D} h \right]
e^{-\sigma \mathcal{A}} \right]_{\mbox{\tiny{up to first order}}}
\en
The Taylor expansion of the exponent gives:
\eqa\label{sigmaa}
\sigma \mathcal{A} \simeq & &\!\!\!\!\!\!\!\! \sigma RL + \frac{\sigma}{2}
\int_0^R \!\!\! dz \int_0^L \!\!\! dt 
\left[ \left( \frac{\partial h}{\partial z} \right)^2 \!\!\!
+\left( \frac{\partial h}{\partial t} \right)^2 \right] \nonumber \\ 
& & + \frac{\sigma b}{4} \int_0^L \!\!\! dt
\left[  \left( \frac{\partial h}{\partial z} \right)_{z=0}^2 \!\!\!\!
+  \left( \frac{\partial h}{\partial z} \right)_{z=R}^2
\right]
\ena
We can think about this formula as the starting point
in a perturbative analysis in terms of the $b$
parameter, namely we
can consider the boundary term as a perturbation
of the pure Nambu--Goto action Eq. (\ref{nambugoto}).\\
First of all, let us notice that:
\begin{enumerate}
\item by virtue of the fact that the eigenvalues
of the unperturbed problem are known --- see
Eq. (\ref{autovalori-lapl}) --- the double integral appearing in 
Eq. (\ref{sigmaa}) can be written in a simpler way:
\eqa
\label{duezampe}
\int_0^R \!\!\! dz \int_0^L \!\!\! dt 
\left[ \left( \frac{\partial h}{\partial z} \right)^2 \!\!\!
+\left( \frac{\partial h}{\partial t} \right)^2 \right] =
\nonumber \\
= \pi^2 \left( \frac{n^2}{\rho^2} + \frac{m^2}{\tau^2} \right)
\cdot \int_0^R \!\!\! dz \int_0^L \!\!\! dt 
\left( \dots \right)_{[z,t]^2}
\ena
where the notation $\left( \dots \right)_{[z,t]^2}$ 
represents (the square modulus of) the complete,
unperturbed eigenfunction.
\item On the other hand, Eq. (\ref{autovaloriin0er}) shows 
that the two addends 
appearing in the integral associated to the
boundary term in Eq. (\ref{sigmaa}) are equal, and 
they give rise to a contribution which can be 
written as:
\eqa\label{unazampa}
\int_0^L \!\!\! dt
\left[  \left( \frac{\partial h}{\partial z} \right)_{z=0}^2 \!\!\!\!
+  \left( \frac{\partial h}{\partial z} \right)_{z=R}^2
\right] = \nonumber \\
= 2 \frac{n^2 \pi^2}{R^2} \cdot \int_0^L \!\!\! dt
\left( \dots \right)_{[t]^2}
\ena
In this case, the integrand $\left( \dots \right)_{[t]^2}$
is just (the square modulus of) the $t$-dependent
part of the
eigenfunction\footnote{The
$z$-dependence does not appear, because we already 
evaluated its value in $z=0$ and in $z=R$.}.
\end{enumerate}
Thus, in the ``pure Nambu--Goto'' case,
$\sigma \mathcal{A}_0$ involves terms like:
\eq\label{terminipurenambugoto}
\frac{\sigma}{2} \pi^2 \left( \frac{n^2}{\rho^2} + \frac{m^2}{\tau^2} \right)
\cdot \int_0^R \!\!\! dz \int_0^L \!\!\! dt 
\left( \dots \right)_{[z,t]^2}
\en
but when the boundary term is included this
expression has to be replaced by:
\eq\label{terminicompleta}
\frac{\sigma}{2} \pi^2 \left( \frac{n^2}{\rho^2} + \frac{m^2}{\tau^2} \right)
\cdot \int_0^R \!\!\! dz \int_0^L \!\!\! dt 
\left( \dots \right)_{[z,t]^2} + \frac{\sigma b}{2}
\frac{n^2 \pi^2}{R^2} \cdot \int_0^L \!\!\! dt
\left( \dots \right)_{[t]^2}
\en
The integrals appearing in Eq. (\ref{terminicompleta})
give rise to results\footnote{The results appearing in
Eq. (\ref{nonnormalizzata2}) and Eq. (\ref{nonnormalizzata1})
refer to an unnormalized
eigenfunction, but this is not relevant to our present
calculation, since the only difference in the normalized
eigenfunction case is that both quantities are 
multiplied by a common factor, and their ratio is
unchanged.} in the form:
\eqa
\label{nonnormalizzata2} 
\int_0^R \!\!\! dz \int_0^L \!\!\! dt 
\left( \dots \right)_{[z,t]^2} &=& C_2 \cdot RL \\
\label{nonnormalizzata1}
\int_0^L \!\!\! dt
\left( \dots \right)_{[t]^2} &=& C_1 \cdot L
\ena
where $C_2$ and $C_1$ are just pure numbers\footnote{Strictly 
speaking, this is true only if we do not consider
the usual normalization factor; however, even in the
more general case, the ratio between $C_2$ and $C_1$
will be the same as we find here.}; thus we can rewrite 
Eq. (\ref{terminicompleta}) as:
\eqa
\label{conglobare}
& & \sigma \frac{\pi^2}{2} \left( \frac{n^2}{\rho^2} + \frac{m^2}{\tau^2} \right)
\cdot C_2 RL + \frac{\sigma b}{2}\pi^2
\frac{n^2}{R^2} \cdot C_1 L = \nonumber \\
& & = \sigma RL \frac{\pi^2}{2}C_2 \cdot 
\left[ \left( \frac{n^2}{\rho^2} + \frac{m^2}{\tau^2} \right) +
\frac{b}{R} \cdot \frac{C_1}{C_2} \cdot \frac{n^2}{\rho^2} 
\right] 
\ena
Defining:
\eq\label{k}
k=\frac{C_1}{C_2}
\en
then Eq. (\ref{conglobare}) can be rewritten as:
\eqa
\label{riscritturacompleta}
& & \sigma \frac{\pi^2}{2} \cdot C_2 RL \left[
\frac{m^2}{\tau^2} + \frac{n^2}{R^2} \left(
1 + k \frac{b}{R}
\right) \right] = \nonumber \\
& & = \sigma \frac{\pi^2}{2} \cdot C_2 RL \left\{
\frac{m^2}{\tau^2} + \frac{n^2}{\left[
R \left( 1 + k \frac{b}{R} \right)^{-\frac{1}{2}}
\right]^2} \right\}
\ena
By defining:
\eq\label{rstar}
R^\star = R \left( 1 + k \frac{b}{R} \right)^{-\frac{1}{2}}
\en
Eq. (\ref{riscritturacompleta}) takes the form:
\eq
\label{esattamenteuguale}
\sigma \frac{\pi^2}{2} \cdot C_2 RL \left(
\frac{m^2}{\tau^2} + \frac{n^2}{{R^\star}^2}
\right)
\en
In the pure Nambu--Goto theory (with no boundary term),
the corresponding term:
\eq
\label{corrispondente}
\sigma \frac{\pi^2}{2} \cdot C_2 RL \left(
\frac{m^2}{\tau^2} + \frac{n^2}{R^2}
\right)
\en
is associated to the $Z_1$ term in the partition function
factorization formula Eq. (\ref{z0+1}); in three dimensions,
$Z_1$ turns out to be equal to:
\eq\label{z1}
Z_1 = \left[ \eta \left( i \frac{\tau}{\rho} \right) \right]^{-1}
= \left[ \eta \left( i \frac{L}{2R} \right) \right]^{-1}
\en
and its (additive) contribution to the interquark
potential is:
\eq\label{v1}
V_1(R) = - \frac{1}{L} \log Z_1 = \frac{1}{L} \log \eta \left( i \frac{L}{2R} \right)
\en
Since Dedekind's function is defined as:
\eq
\label{eta}
\eta \left( i \frac{\tau}{\rho} \right) = q^\frac{1}{24}
\prod_{n=1}^{+\infty} (1-q^n) \;\;\;\;\; , \;\;\;\;\;
q=e^{-2\pi \frac{\tau}{\rho}}
\en
In the regime $\frac{L}{2R} \gg 1$, we can approximate:
\eqa \label{luescherterm}
V_1(R) \!\!\!\!\!\!\!\! & & = \frac{1}{L} \left[
-\frac{\pi L}{24 R} + \sum_{n=1}^{+\infty} \log
\left( 1 - e^{-\frac{\pi L}{R}n} \right)
\right] \simeq \nonumber \\
& & \simeq - \frac{\pi}{24 R}
\ena
which is nothing but the celebrated
``L\"uscher term'' \cite{lsw}.\\
When the boundary term is included in the action,
we get a similar result, provided we replace:
\eq\label{sostituzione}
R \longrightarrow R^\star = R \left( 1 + k \frac{b}{R} \right)^{-\frac{1}{2}}
\en
We can evaluate $k$ in simple way: its definition is given by
Eq. (\ref{k}), which involves the integrals in
Eq. (\ref{nonnormalizzata2}) and in
Eq. (\ref{nonnormalizzata1}), thus:
\eqa
\label{calcolokparte1}
k=\frac{C_1}{C_2}=R \cdot
\frac{\int_0^L \!\!\! dt
\left( \dots \right)_{[t]^2}}{\int_0^R \!\!\! dz \int_0^L \!\!\! dt
\left( \dots \right)_{[z,t]^2}}
\ena
Since the two eigenfunction parts expressing the
$t$-dependence and $z$-dependence are factorized, the denominator
integrals factorize, too. Moreover, we know that the
$z$-dependent part of the eigenfunction is
expressed by Eq. (\ref{zdependence}); these observations allow
one to write:
\eq
\label{calcolokparte2}
k= R \frac{\int_0^L \!\!\! dt 
\left( \dots \right)_{[t]^2}}{ \int_0^R
\sin^2 \left( \frac{n\pi z}{R}
\right)
\int_0^L \!\!\! dt 
\left( \dots \right)_{[t]^2}} =
R \cdot \frac{1}{\frac{1}{2} \; R} = 2
\en
where we exploited the fact that $n \in \mathbf{N}_0$.\\
Thus, in the case when we allow for the presence of 
the boundary term, the first-order non-trivial 
contribution to the interquark
potential will be:
\eq\label{v1staresatto}
V_1^\star = 
\frac{1}{L} \log \eta \left( i \frac{L}{2R^\star} \right)
\en
It is important to stress the fact that this result does not
rely on the assumption to be in the ``large $\frac{L}{2R}$
regime'': as a matter of fact, the only hypothesis 
for the validity of Eq. (\ref{sostituzione}) is that
$b$ can be considered as a perturbatively small parameter.\\
On the other hand, if we restrict to the case
when $\frac{L}{2R} \gg 1$, then Eq. (\ref{v1staresatto})
can be approximated by:
\eqa\label{v1starapprossimato}
V_1^\star \!\!\!\!\!\!\!\!& & \simeq - \frac{\pi}{24 R^\star} = - \frac{\pi}{24 R \left( 1 + 
2 \frac{b}{R} \right)^{-\frac{1}{2}}} = \nonumber \\
& & = - \frac{\pi}{24 R} \sqrt{ 1 + 2 \frac{b}{R} }
\simeq - \frac{\pi}{24 R} \left( 1 + \frac{b}{R}  \right)
\ena
which exactly reproduces the term appearing in Eq. (3.9) in
\cite{lw02}.

